Cryptomining Makes Noise: a Machine Learning Approach for Cryptojacking Detection

A new cybersecurity attack,where an adversary illicitly runs crypto-mining software over the devices of unaware users, is emerging in both the literature and in the wild . This attack, known as cryptojacking, has proved to be very effective given the simplicity of running a crypto-client into a target device. Several countermeasures have recently been proposed, with different features and performance, but all characterized by a host-based architecture. This kind of solutions, designed to protect the individual user, are not suitable for efficiently protecting a corporate network, especially against insiders. In this paper, we propose a network-based approach to detect and identify crypto-clients activities by solely relying on the network traffic, even when encrypted. First, we provide a detailed analysis of the real network traces generated by three major cryptocurrencies, Bitcoin, Monero, and Bytecoin, considering both the normal traffic and the one shaped by a VPN. Then, we propose Crypto-Aegis, a Machine Learning (ML) based framework built over the results of our investigation, aimed at detecting cryptocurrencies related activities, e.g., pool mining, solo mining, and active full nodes. Our solution achieves a striking 0.96 of F1-score and 0.99 of AUC for the ROC, while enjoying a few other properties, such as device and infrastructure independence. Given the extent and novelty of the addressed threat we believe that our approach, supported by its excellent results, pave the way for further research in this area.

==> mod.tex <==
1.	Contributions Statement.

While the author claims in the ‘ABSTRACT’ section to have made 5 contributions, it might be difficult for a reader to appreciate and recognize some of them. E.g. while mentioning ‘(i) We identify and model a new type of attack, i.e., the sponge-attack, being a generalization of cryptojacking’, the author does not explicitly state the difference (or generalization) with the cryptojacking attack they are considering. 
Apart from that, I believe, the ‘(v) We compare our results against competing solutions in the literature’ still refers to the contribution mentioned previously – the development of the framework in general. 
On the other hand, the ‘INTRODUCTION’ section states the twofold contribution, which compromises consistency in the contributions formulation in general. 

2.	Framework Description. 

The formulation of the Crypto-Aegis framework capabilities and objectives appear to be different across the article. 
‘ABSTRACT’ states that the framework can ‘detect and identify clients suffering from a sponge-attack’. Later in‘TRAFFIC CLASSIFICATION: A BASELINE EXAMPLE.’ (please also note that this subtitle has a dot in the end, while the others do not) the author mentions: 'In this section, we introduce a simplified version of our methodology considering a binary decision problem with the aim of discriminating a stealthy miner from the network traffic generated from an office laptop.' 
I believe the ambiguity of these definitions may cause confusion about the framework’s facilities. 
Apart from that, later on, the framework even demonstrated the ability to identify the exact cryptocurrency the attacking client belongs to, which, I believe, was not mentioned before. 

3.	Reference Issues.

References [10] and [11] seem to be the same work referenced at different parts of the article. The reference format also appears to be inconsistent. 
%MC: References [10] and [11] are different in the paper submitted to ASIACCS. The comment seems not true

4.	Terms Definitions.

4.1. Several terms throughout the whole article are introduced before they are explained. E.g. the term ‘Crypto-client’ is used 9 times before it is introduced. While that can be explained by the fact that this term appears since the very beginning of the article, ‘Interarrival time’ measurements, for example, are provided and discussed several times in the ‘NETWORK TRAFFIC ANALYSIS AND PATTERNS’ before the definition is provided.
%MC: each occurence of "Crypto client" replaced with "Crypto-client"
%MC: Consider moving Section III.C (Terminology)
4.2. On the other hand, the article contains 2 definitions of terms ‘Full-Node’ and ‘Master’ in ‘Scenario’ and ‘Full Node Vs Miner’ subsections respectively.
%MC: Fixed

5.	Experiments Description

5.1. In ‘MEASUREMENT SETUP AND PRELIMINARY CONSIDERATIONS’ the author provides the reader with the information about the model of the laptop being used as a reference device in the experiments, while I would have suggested to specify its technical characteristics as a more informative scale. %MC: Anche no

5.2. While the author provides the accuracy statistics (True Positive and False Positive Rates) for both their framework (in sections 6-8) and other solutions (in ‘RELATED WORK’) separately, I find it to be very illustrative if they would have compared those results in one table (for a similar and comparable functionality, e.g. ‘Miner Detection’).

6.	Subtitles and Their Order.

6.1. The sections presenting the experiments’ outcome are provided in the following order: ‘CRYPTO-AEGIS: DETECTION AND IDENTIFICATION OF FULL NODES’, ‘CRYPTO-AEGIS: DETECTION AND IDENTIFICATION OF MINERS’ and ‘CRYPTO-AEGIS: SPONGE-ATTACK DETECTION ’. If I understand properly, the last one appears to be the generalization of the first two. Therefore, I would have proposed to consider the logical movement from general to specific, instead of the opposite.  %MC: non sono d'accordo

6.2. Apart from that, ‘CRYPTO-AEGIS: DETECTION AND IDENTIFICATION OF FULL NODES’ contains the following sentence: ‘Our results prove that ... can be used to effectively identify malicious miners inside local networks.’ As this subsection is dedicated to Full-Nodes’ identification (not miners’) the terminology may seem inconsistent.

7.	Wording.

7.1. There is some inconsistency in using both ‘adversary model’ and ‘adversarial model’ phrases, even in the subtitles. I believe the term ‘adversary model’ is the one being normally used in this context.
%MC: Fixed

7.2. In ‘TRAFFIC CLASSIFICATION: A BASELINE EXAMPLE.’ the author provides the following statement:
‘Firstly, we observe that, for this scenario — Bitcoin Vs Office — the most important feature is γ, i.e., the packet size, represented by the red bar. The other features have about the same weights, ...’
I would like to recommend to review this formulation, as, I believe, saying ‘the same weights’ in this context means ‘same weights as the most important feature has’, while there is a chance that what is really being meant is ‘other weights have the equal weights’. %non ho capito

7.3. In ‘CRYPTO-AEGIS: DETECTION AND IDENTIFICATION OF FULL NODES’ the author says:
‘Misclassifications [of Bytecoin crytpo-clients] are mainly due to Monero’.
Saying ‘due to’ in the context of misclassification can be quite misleading for a reader. From the context, it is understandable that the crypto-client class name provided after ‘due to’ stands for the crypto-client class the real one is confused with, instead of the reason for that confusion. It also is repeated for several times across the paper.

7.4. ‘RELATED WORK’ states the following:
‘Dedicated small devices (e.g., smartphones, laptops, desktop), or more powerful ones (e.g., workstations, servers), to the mining process would not be worth the cost of the electricity.’
I assume that what was meant to be compared with the cost of electricity is the contribution of the non-specialized devices to the mining process, instead of the devices themselves.

7.5. Some of the conclusions appear to be hardly derivable to me. E.g. the following statement from the ‘INTRODUCTION’ section:
‘Indeed, both the crypto-currencies adopt the CryptoNight hash function where the marginal benefit derived from specialized architectures such as GPU, FPGA, or ASIC does not introduce any significant gain for justifying the adoption of such as hardware. Therefore, mining is usually performed via CPU-based architectures.’ 
Even though I understand that in the last sentence the author talks about only CPU-mineable cryptocurrencies, it may sound like they spread this assumption to all the other cryptocurrencies.

7.6. The word ‘indeed’ appears 16 times in the paper, which is more often than one time per page. 

7.7. The article may also be reviewed from the point of grammar and language.
E.g., 'A Russian nuclear scientists has been arrested', 'Miners detection performance are similar', small ‘n’ in ‘new Zealand’ in the name of the conference is the header.

